Tight Bounds for Online Edge Coloring

Vizing's celebrated theorem asserts that any graph of maximum degree $\Delta$ admits an edge coloring using at most $\Delta+1$ colors. In contrast, Bar-Noy, Naor and Motwani showed over a quarter century that the trivial greedy algorithm, which uses $2\Delta-1$ colors, is optimal among online algorithms. Their lower bound has a caveat, however: it only applies to low-degree graphs, with $\Delta=O(\log n)$, and they conjectured the existence of online algorithms using $\Delta(1+o(1))$ colors for $\Delta=\omega(\log n)$. Progress towards resolving this conjecture was only made under stochastic arrivals (Aggarwal et al., FOCS'03 and Bahmani et al., SODA'10). We resolve the above conjecture for \emph{adversarial} vertex arrivals in bipartite graphs, for which we present a $(1+o(1))\Delta$-edge-coloring algorithm for $\Delta=\omega(\log n)$ known a priori. Surprisingly, if $\Delta$ is not known ahead of time, we show that no $\big(\frac{e}{e-1} - \Omega(1) \big) \Delta$-edge-coloring algorithm exists. We then provide an optimal, $\big(\frac{e}{e-1}+o(1)\big)\Delta$-edge-coloring algorithm for unknown $\Delta=\omega(\log n)$. Key to our results, and of possible independent interest, is a novel fractional relaxation for edge coloring, for which we present optimal fractional online algorithms and a near-lossless online rounding scheme, yielding our optimal randomized algorithms.

==> algorithm.tex <==
\section{The Bounded Water filling with Fractional Algorithm}\label{sec:fractional}\dwnote{fix title}
In this section, we describe our online fractional coloring algorithm for 
bipartite and general graphs. Our algorithms are both instances of a more general edge coloring algorithm we provide, only differing in the choice of the bound parameter $\beta$.
Given a graph $G(V,E)$, the fractional relaxation of the edge coloring problem is as follows. A graph is (fractionally) $\Delta$-edge-colorable, if there is a feasible solution to the linear program
\begin{align*}
\sum_{c = 1}^{\Delta} x_{e,c} &= 1  \qquad \qquad \forall e \in E\\
\sum_{e: u \in e} x_{e,c} &\leq 1 \qquad \qquad \forall v\in V, c \in \Delta \\
x_{e,c} &\geq 0 \qquad \qquad  \forall e\in E, c \in \Delta
\end{align*}

It easy to verify that the minimal number of colors $\Delta$ is equal to the maximal degree of a vertex in the graph. For notational simplicity, rather than discussing fractional algorithms using some $\alpha \cdot \Delta$ colors, we will instead use $\Delta$ colors and relax the second constraint to 
\begin{align*}
\sum_{e: u \in e} x_{e,c} &\leq \alpha \qquad \qquad \forall v\in V, c \in \Delta
\end{align*}
Because we are dealing with fractional solutions, it is easy to ``stretch'' such a solution to obtain a feasible edge coloring (i.e., satisfying $\sum_{e: u \in e} x_{e,c} \leq 1$) while using $\lceil\alpha \cdot \Delta\rceil \leq \alpha\cdot \Delta + 1$ colors, and this can be done online.
%There is a one-to-one correspondence to a solution which uses $\alpha \cdot \Delta$ colors (up to an additive constant).
Therefore, our goal is to bound $\alpha$ -- the competitive ratio.

In the algorithm, upon arrival of a new vertex $v$, we run a variant of the water filling algorithm on each edge $(u,v)$ in an arbitrary order. The water filling is with respect to the current load of the colors of previously-arrived neighbor $u$, where the load on $u$ of color $c$ is $L_u (c) \triangleq \sum_{e\ni u} x_{e,c}$. 
The main difference compared to the water filling algorithm is that we set up a bound constraint of $\beta/\Delta$ for each color per edge, where $\Delta$ is the \textbf{current} maximal degree, and $\beta$ is a parameter of the algorithm which will be determined later. The bound constraints result in a more balanced allocation, which uses more colors for each edge.
%A formal description of our algorithm is shown in \ref{alg:cap_water_filling}. In the algorithm, upon arrival of a new node $v$, we color its adjacent edges in arbitrary order. When deciding the coloring of its adjacent edge $e = (u, v)$, we look at the fractional coloring  of the edges of $v$, or alternatively, the 'load' on coordinate $u$ of each color bin. We run water filling algorithm on these coordinates, with the constraints that increase in each coordinate can be no more than $\beta/\Delta$, where $\Delta$ is \textbf{current} max degree and $\beta$ is a parameter of the algorithm. 


A formal description of our algorithm is shown in \Cref{alg:cap_water_filling}. (Our algorithm is described as a continuous process, but can be easily discretized.)


%\eat{
%\subsection{Preliminary}
%First, we introduce the notation for the algorithm that we will use in the proofs for bipartite graphs as well as for general graphs. 
%We use $\delta_{u}^t$ to refer the global maximum degree when node $u$ has its $t$'th neighbor. Let $A_u$ to denote the degree of $u$ when it arrives. 
%Water filling algorithms preserve important monotone structure on the `load'.  
%Note that our algorithm is asymmetric with respect to the newly arrived vertex, and its already arrived neighbors. But after a vertex $u$ arrives, then all its future edges would be colored with respect to $u$ current fractional colors load, and therefore the monotone load properties would hold with respect to the sorted color load, \textbf{after} the arrival of $v$. 
%Hence, for each vertex $u$ we define an order permutation $o_u: Z^+ \rightarrow Z^+$.
%Where $o_u(i)$ is the index of $u$'s most loaded color index \textbf{after} vertex $u$ arrival, and $o_u(i) = i$, for $i > d^{A_u}_u$. We denote $o^{*}_u$ as the inverse permutation, i.e. $o_u^{*}(o_u(i)) = i$. . \icnote{In the paper we will use color $i$ to refer to $o_u(i)$}
%}

\dwnote{$\Delta_u$ undefined!!!}
\begin{algorithm}[H] 
	\caption{Bounded Water Filling}
	\label{alg:cap_water_filling}

	\begin{algorithmic}[1]
		\Require Online graph $G(V,E)$ with vertex arrival, parameter $\beta\,\,(1 < \beta < 2)$\;
		
		\Ensure Fractional edge coloring $x_{e,c} \in [0,1]$, for $e\in E$, $c\in [\Delta]$ 
		
		
		\For{each arrival of a vertex $v$}
			\State $\Delta = \max\limits_{u\in V} {\Delta_{u}}$. \label{line:delta-init}
			\For{each $(v,u) \in E$}
				\For{all $c\in [\Delta]$}
				\State set $f_{e,c} \leftarrow 0$.
				\EndFor
				\While{$\displaystyle\sum_{i = 1}^{\Delta}f_{e,i} < 1$}
				
				\State let $\mathit{UnSat} \triangleq  \{c \in \Delta \mid f_{e,c} < \beta/\Delta\}$.
				\State let $\mathit{Active} \triangleq \{c \in \mathit{UnSat} \mid L_u(c) = \displaystyle\min_{c\in \mathit{UnSat}} L_u(c)\}$.
				\State increase $f_{e,c}$ continuously, $\forall c \in \mathit{Active}$. \Comment{update $L_u(c),L_v(c)$,$\mathit{UnSat}$ and $\mathit{Active}$.}
								
				\EndWhile
				
%				\For{all $i\in [\Delta]$}
%				\State $\ell^{d_u}_v(i) \leftarrow {\ell}_{u}(i)$.
%				\EndFor
%				\State set the order permutation $o_v$, according to $v$'s current load.
%				\For{all $i\in [\Delta]$}
%				\State $\ell^{d_u}_u(i) \leftarrow {\ell}_u(i)$.
%				\EndFor
%				\For{all $i\in [\Delta]$}
%				\State $\ell_v(i) \leftarrow \ell_v(i) + {\ell}^{d_u}_u(i)-\ell^{d_u-1}_u$.
%				\EndFor
%				\For{all $i\in [\Delta]$}				
%				\State $f_{(v,u)}(i) \leftarrow {\ell}^{d_u}_u(o_u(i))-\ell^{d_u-1}_u(o_u(i))$.
%				\EndFor
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}


\dwnote{The algorithm needs a different notation for $\Delta$. Also $\Delta_u$ was never defined}

==> rounding.tex <==
\section{Rounding Fractional Edge Colorings Online}\label{sec:round}
In this section we show how to round our optimal online fractional edge-coloring algorithms for bipartite graphs. We start by formally defining what it means to round a fractional edge coloring online, and similarly for fractional matching.
%We start with the known-$\Delta$ case, where the fractional algorithm is trivial ($\frac{1}{\Delta}$ for each edge-color pair), and later explain the more general approach. Before either of these, we formally define what online rounding algorithms for fractional edge coloring and matching are.

\begin{Def}
	An \emph{online edge coloring rounding algorithm} (\roundEC) receives as input a fractional edge coloring in an online fashion. Specifically, upon arrival of vertex $v$ the values $f_{e,c}$ for each edge-color pair $(e,c)$ with $e\ni v$ are revealed. The \roundEC then decides immediately and irrevocably which edges of $v$ to color by what color. The choices of an \roundEC following a vertex arrival are called a \emph{\round}.
	\\
	An \emph{online matching rounding algorithm} (\roundM) is defined similarly with respect to online matching.\dwnote{would be nice to say it's a special case of \roundEC, but currently not true for the above definition.}
\end{Def}

At a high level, one cannot expect to round matchings or coloring in a lossless manner either for matchings or for edge colorings, as the $1-O(1/\sqrt{d})$ lower bound of \cite{cohen2018randomized} for online matching in $d$-regular graphs shows.\footnote{For the implication to edge colorings, notice that the fractional solution of $1/d$ for each edge-color pair is feasible for $d$-regular graphs, but coloring with less than $d+o(\sqrt{d})$ colors implies that an average matching size among the color classes matches a $1-o(1/\sqrt{d})$ fraction of the vertices, and as such randomly picking a color class would yield a matching of size surpassing this lower bound.} In fact, this lower bound even shows that one cannot avoid losing a constant multiplicative term when rounding flows of high value. In our case, however, we will have as input fractional solutions have rather low value everywhere, say at most $1/\Delta$.\dwnote{@Ilan, do we have a lemma for this? I can't figure out anything from this notation...} We will rely on this property of our fractional algorithms in order to guarantee concentration in our \roundEC, which we now describe.

\subsection{Our Approach} 
Our \roundEC works as follows. Let $c_{\max}$ be the highest color for which the fractional solution will have some $f_{e,c_{\max}}$ which is non-zero for some edge $e$. (As we will consider only 
bounded-competitive fractional solutions, such a finite $c_{\max}$ exists.)
Upon arrival of an online vertex $v$, we  round the values of all $f_{e,c_{\max}}$ 
values for all $e\ni v$ by applying the next \round of an \roundM on $f_{e,c_{\max}}$. Let $M_{c_{\max}}$ be the matching obtained by the \roundM's 
rounding and let $G=G_{c_{\max}}$. Then, for color $c=c_{\max}-1,c_{\max}-2,\dots,1$, we set 
$G_{c} = G_{c+1} \setminus M_{c+1}$ and run the next \round of the \roundM on $f_{e,c}$ restricted to the edges in $G_{c}$. Finally, we color all uncolored edges $e$ (i.e., $e \not \in \bigcup_{c=1}^{c_{\max}} M_c$) greedily, with a different set of colors labeled $-1,-2,\dots$.

For our \roundEC to obtain bounded competitive ratio, we rely on an \roundM 
which matches each edge with probability roughly equal to the marginals prescribed by the fractional matching which the \roundM receives as input. This 
will imply that after some $k$ colors' fractional matching are rounded by this \roundM each vertex $v$ (online or offline) will have its degree decrease in expectation by at least $\approx\sum_{e\ni v} \sum_{c=c_{\max}-k+1}^{c_{\max}} f_{e,c}$.
By standard concentration bounds, we expect that following the rounding of the $c_{\max}$ fractional matchings, each vertex $v$ should have a $U(v)$, its number of unmatched neighbors, close to its expectation; i.e., close to zero. The following greedy matching would then incur a small additive term.

The above approach seems nice and simple, but we quickly run into the following issue: an edge which is colored with some color $c$ by the \roundEC will no longer be available for the \roundM. This, in particular decreases the expected number of edges of a given vertex $v$ matched in the lower-numbered colors. To circumvent this difficulty we need to \emph{increase}
the values $f_{e,c}$. But how can we do this without violating the fractional matching constraints, without which the \roundM is not guaranteed to work? Here we rely again on concentration bounds (now relying on edges not being matched with probability above their fractional value) to argue that a per-edge multiplicative increase after every $o(\Delta)$ colors yields a feasible fractional matching with high probability while also roughly maintaining $f_{e,c}$ in expectation when $e$ is not colored by some higher color; i.e., guaranteeing 
$\mathbb{E}[f_{e,c}\cdot \mathds{1}[e\not \in \bigcup_{c+1}^{c_{\max}} ] ] \approx f_{e,c}.$ We then find that the fact that we only round the values once every $o(\Delta)$ colors incurs an additional $o(1)$ loss in our marginal probabilities of matching each edge, and overall we find that each edge is colored with probability $1-o(1)$ over all colors. This time applying to concentration inequalities, we finally find that the \roundEC only requires some $o(\Delta)$ more colors than the fractional edge coloring it receives as input.

\subsection{Our Algorithm}
Here we give our \roundEC algorithm, \Cref{alg:round-ec}, below.

\begin{algorithm}[H] 
	\caption{\roundEC for bipartite vertex arrival}
	\label{alg:round-ec}
	
	\begin{algorithmic}[1]
		\Require Online bipartite graph $G(L,R,E)$ and fractional edge coloring $\{f_{e,c} \mid e,c\}$, $f_{e,c} \leq o(1)$ $\forall e,c$.
		
		\Ensure Integral edge coloring using the same number of colors as $f$ plus $o(\Delta)$, w.h.p.
		
		\For{each color $c$, implicitly}
		\State set $G_c\leftarrow G$ and $M_c \leftarrow \emptyset$.
		\EndFor 
		
		\For{each arrival of a vertex $v\in R$}
		\For{each color $c$ with non-trivial $\vec{f}^{(c)}$, in decreasing order of $c$}
		\State run one \round of \roundM on $\vec{f}^{(c)}$ restricted to $G_{c}$. 
		\If{some edge $e$ is matched by the \roundM above}
		\State set $M_c \leftarrow M_c \cup \{e\}$.
		\EndIf
		\State set $G_{c-1} \leftarrow G_c \setminus M_c$.
		\If{$c$ satisfies some numeric condition} 
		\For{each color $c'\in [c-1]$} 
		\State $\textrm{Update}(\vec{f}^{(c')},f)$ \Comment{condition and transformation to be formalized}
		\EndFor
		\EndIf
		\EndFor
		\EndFor
		\State run greedy on all edges still uncolored (i.e. $e\in E\setminus \bigcup_{c=1}^{\infty} M_c$), using colors $-1,-2,\dots$. \label{line:greedy}
	\end{algorithmic}
\end{algorithm}

\dwnote{Fill in missing details in algorithm.}

To make \Cref{alg:round-ec} a concrete algorithm, we must specify when and how we update fractional matchings. First, we note that we must somehow increase the values of $\vec{f}^{(c')}$, as the following example illustrates. For simplicity (though this is too good be true in general), we assume that our \roundM matches each edge $e$ with probability \emph{precisely} $1/\Delta$ in $M_c$ if $e\in G_{c}$. Consider a star graph of degree $\Delta$, with the star's center arriving last and  each edge-color pair  assigned value $f_{e,c}=1/\Delta$. Denote by $p_{e,c} = \Pr[e\in M_c]$ the probability that $e$ is colored $c$ and by $P_{e,c} = \sum_{c'> c} p_{e,c'}$ the probability that $e$ is colored by a higher color than $c$. Then, we find that if we do not increase the $f_{e,c}$ in some way in our algorithm, the probabilities $p_{e,c}$ satisfy the recurrence relation
\begin{align*}
	p_{e,c} = \frac{1}{\Delta} \cdot (1-P_{e,c}) = \frac{1}{\Delta}\cdot \left(1-\sum_{c'>c} p_{e,c'}\right).
\end{align*}
But this recurrence captures non-empty bins in a balls and bins process with $\Delta$ balls (colors) thrown into $\Delta$ bins (edges). Specifically, $p_{e,c}$ corresponds to an indicator for $c$ being the first ball occupying bin $e$. The expected number of non-empty bins in the above process, $\sum_c p_{e,c}$, tends to $(1-\frac{1}{e})\Delta$ as $\Delta$ grows, and so $\frac{\Delta}{e}+o(\Delta)$ edges are not matched before \Cref{line:greedy}. Consequently, our algorithm would use at least $(1+\frac{1}{e}-o(1))\cdot \Delta = (1+\Omega(1))\cdot \Delta$ colors on this star of maximum degree $\Delta$.

Motivated by the above, we strive to update the values in $f^{(c)}$ after rounding $\vec{f}^{(c+1)}$ by setting
\begin{equation}\label{update-ideal}
	\textrm{updated}(f_{e,c}) = \begin{cases} 
	f_{e,c}/(1-P_{e,c}) & e \not\in \bigcup_{c' > c} M_{c'} \\
	0 & \text{else}.
	\end{cases}
\end{equation}
\dwnote{Define something for uncolored, instead of $\left[e\not\in \bigcup_{c'\geq c}M_{c'}\right]$}
If we update the values this way the expected value of this updated $f_{e,c}$ is precisely 
\begin{equation}\label{update-ideal-marginals}
(f_{e,c}/(1-P_{e,c})) \cdot \Pr\left[e\not\in \bigcup_{c'\geq c}M_{c'}\right] = (f_{e,c}/(1-P_{e,c})) \cdot (1-P_{e,c}) = f_{e,c}.
\end{equation}

Updating the $f_{e,c}$ values as in \eqref{update-ideal} is difficult, however, as we will not have a closed-form expression for $P_{e,c}$ for our algorithm. Instead, we settle for an upper bound $\widehat{P_{e,c}}$ for this $P_{e,c}$ satisfying 
\begin{equation}\label{p-estimate}
1-P_{e,c} \leq 1-\widehat{P_{e,c}} \leq (1-P_{e,c})/(1-\epsilon)
\end{equation} 
for some small $\epsilon$. 
A bound satisfying \eqref{p-estimate} w.h.p.~is easily obtained by monte-carlo methods,\dwnote{can get exponentialy-small error, so can ignore} by running our algorithm some $\poly(n,\log(\epsilon^{-1}))$ times on the prefix of the input so far and using the fraction of times the edge $e$ was matched by the colors $c'> c$, shifted slightly, as an estimate. The advantage of updating $f_{e,c}$ using such an estimate is that now the expected updated value, while not exactly equal to $f_{e,c}$, is at most some $1/(1-\epsilon)$ multiplicative term smaller.

\begin{lem}
	Let $\widehat{P_{e,c}}$ be as in \eqref{p-estimate}. Then, replacing $P_{e,c}$ by $\widehat{P_{e,c}}$ in \eqref{update-ideal}, we obtain 
%	$\textrm{\emph{updated}}(f_{e,c}) = f_{e,c}/(1-\widehat{P_{e,c+1}})$, we obtain
	\begin{equation}
		\E\left[\textrm{\emph{updated}}(f_{e,c})\right] \in [f_{e,c}\cdot (1-\epsilon), f_{e,c}].
	\end{equation}
\end{lem}

In particular, as our \roundM loses only a $o(1)$ multiplicative term compared to the updated value $f_{e,c}$ when $e$ is uncolored, we find that in expectation we should only lose some $\epsilon + o(1)$ multiplicative term compared to $f_{e,c}$. We would therefore expect to match all but at most some $\Delta(\epsilon + o(1)))$ edges of each vertex. If we can guarantee $\epsilon=o(1)$, we should be able to argue concentration of measure and therefore each vertex should have few -- specifically, some $o(\Delta)$ -- uncolored edges by the time we reach \Cref{line:greedy}, and so this line and our overall algorithm will only require some $o(\Delta)$ colors more than the online fractional solution.\dwnote{To address. Dependence between different color classs. Reason for only updating periodically. Also, no concentration if $\sum_{e\ni v, c} f_{e,c}$ is small, but in that case the degree of $v$ is small, so who cares...}

\subsection{Worries}

\begin{enumerate}
	\item \textbf{Make sure additive error terms are at most 1/number of \metaphase{}s. E.g., if $c^{0.4}$-length \metaphase{}s, can allow for $o(\Delta^{-0.6})$ error, since have $\Delta^{0.6}$ \metaphase{}s.}
	\item \textbf{Make sure multiplicative error terms don't multiply}

	\item updated $f_{e,c}$'s get much larger than $1/c$ (seems OK, if use \Cref{cap-updated})
	\item $o(1)$ terms somehow aggregate exponentially...
	\item \textbf{our rounding algorithm needs to lose something depending on values being small. (No time to write..)}
	\item bounds not in terms of $\Delta$ but rather something like $c$ (though can assume $c\geq \Delta^{5/6}$)....
	\item aggregate all exponents still ok... $(1/3,1/2,5/6...$)
	\item How much do we scale down the values for fractional feasibility after \metaphase{}s?
	\item How ugly is $\Delta = \poly \log n$ term?
\end{enumerate}

\subsection{More stuff}

Of course, the above argument assumed that the rounding of the updated $f_{e,c}$ are independent for different values of $c$, which is clearly false. Instead, we will now rely on the fact that we round \emph{few} (but $\omega(1)$) matchings in between updates of $f_{e,c}$ values. We call the time between updates of these values a \emph{\metaphase}. For a phase starting with color $c$, we will run a \round of our \roundM for the next $\lceil c^{2/3} \rceil$ colors. The interest in these short rounds is that they will allow us to argue concentration w.h.p of the following values for each vertex $v$.
\begin{enumerate}
	\item \label{many-matched} Number of colored edges of $v$ during the \metaphase. 
	\item \label{feasible} $\sum_{e\ni v} f_{e,c'}$ for each color class $c'$ not in the \metaphase after the updates.
\end{enumerate}
\dwnote{Move to section intro?}


The former property, \ref{many-matched}, is useful as it will allow us to argue that if we have some values $\sum_e f_{e,c}$ for a color $c$ in the \metaphase, we expect to color roughly (say, up to some $(1-o(1))$ multiplicative term), some $\sum_{e\ni v} f_{e,c}$ edges of $v$, provided the fractional matching $f^{(c)}$ is feasible. The second property, \ref{many-matched}, will allow us to argue that each fractional matching $f^{(c)}$ remains feasible after an update (which is necessary for our \roundM).

The way we use the relative shortness of the phases to prove properties \ref{many-matched} and \ref{feasible} above can be broadly explained thus. Let $C_{v,c} \triangleq \mathds{1}[\exists e: v\in e\in M_c]$ be an indicator for the event that some edge of $v$ is colored $c$. Note that $\E[C_{v,c}] \approx \sum_{e\ni v} f_{e,c}$, due to our \roundM.
We will argue that the (clearly dependent) variables $C_{v,c}$ for each $c$ in the \metaphase can be lower bounded by independent random variables which have expectation roughly the same as $C_{v,c}$. Applying standard concentration inequalities then yields the following lemma.
\textbf{For our proof of the following lemma.... we will use the follow standard result, easily obtained by a simple coupling argument. We omit the proof for brevity.}

\begin{lem}\label{color-concentration}
	Let $C_{v,c}$ be as above and $S\subseteq \mathbb{Z}$ be the subset of colors of a \metaphase. Then, w.h.p $$\sum_{c\in S} C_{v,c}\geq \E[\sum_{c\in S} C_{v,c}] - O(1/\sqrt{c}).$$
\end{lem}
\begin{proof}
	\dwnote{To do: rewrite without $X_i,Y_i,Z_i$ garbage}
	We appeal to \Cref{lem:coupling} where the $X_i$ and $Y_i$ variables will all be $C_{v,c}$'s. Specifically, we note that for any vertex $v$ and color $c$, conditioning on any realization $\mathcal{R}$ of the $O(c^{2/3})$ variables $\{C_{v,c'} \mid c'>c, c'\in S\}$, we have 
	$$\Pr[C_{v,c} \mid \mathcal{R}]\geq \sum_{e\ni v} f_{e,c} (1-o(1)) - O(c^{-1/3}).$$
	To see this, note that every one of the previous $O(c^{2/3})$ colors in $S$ can result in at most one of $v$'s edges being colored, therefore removing at most $O(1/c)$ from $\sum_{e\ni v, e \text{uncolored}} f_{e,c}$. Therefore, our \roundM will color an edge of $v$ with probability at least 
	\begin{align*}
	[\sum_{e\ni v, e \text{uncolored}} f_{e,c} \mid \mathcal{R}] & \geq \sum_{e\ni v} f_{e,c} - O(c^{2/3} / c) \\
	& = \sum_{e\ni v} f_{e,c} - O(c^{-1/3}).
	\end{align*}
	 \dwnote{Need to assume $f_{e,c}\leq O(1/c)$}
	Now, summing over all the $c^{2/3}$ colors, we have that the independent variables $Z_i$ with the above marginal probability have expected sum $\E[\sum_i Z_i] \geq \sum_{e\ni v} \sum_{c\in S} f_{e,c} - O(c^{1/3})$, which is consistent with the required bound. We then appeal to Hoeffding's inequality to show that these $c^{2/3}$ independent variables have their sum deviate from its mean by at most $O(c^{1/3}\sqrt{\log n}) = O(c^{1/2})$ with high probability. The lemma then follows by \Cref{lem:coupling}.
\end{proof}

\dwnote{intuition} Now, as we will have $\sum_{e\ni v} \sum_{c} f_{e,c}$ maintained in expectation per \metaphase, we will match $\sum_{e,c} f_{e,c}$ .... For this, we need to also prove concentration of $\sum_{e,c} f_{e,c}$ for each \metaphase{}s with high probability. The next lemma does just this, while also implying feasibility of the fractional matchings $f^{(c)}$ after updating of values $f_{e,c}$ at the end of the \metaphase.

\begin{lem}\label{frac-deg-concentration}
	Let $S$ be some set of colors during a \metaphase, starting at color $c$.
	Let $c'=O(c)$ be some color lower than all colors in $S$. \dwnote{generalize. not really what we wrote here...} Then, w.h.p. the fractional matching $\vec{f}^{(c')}$ is feasible after updates at the end of the \metaphase.\textbf{feasible after all metaphases.}
\end{lem}
\begin{proof}
	
	\textbf{NEED TO VERIFY: ADDITIVE ERROR IS AT MOST 1/(NUMBER OF META PHASES).... SPLIT UP LEMMA INTO TWO MAYBE?}\\
	
	\textbf{maybe useful to assume $\sum_{e} B_e$ large?}
	
	\textbf{BE CAREFUL! $c'$ can be as small as $c^{0.9}$.}
	
	\dwnote{TODO: figure out what we need from other lemmas for generalization} 
	
	\dwnote{TODO 2: also note only care about cases where $\sum_{e\ni v} B_e\geq $}
	
	For notational simplicity, let $B_e = f_{e,c'}$, and let $U_e=\mathds{1}[e\not \in \bigcup_{c\in S} M_c]$ be the an indicator for the event that edge $e$ is not colored during the \metaphase.
	Our update values, denoted by $UB_e \leftarrow (B_e/\Pr[U_e]) \cdot U_e$, clearly satisfy
	\begin{equation}\label{frac-deg-exp-bound}
	\E[\sum_{e\ni v} UB_e] = \sum_{e\ni v} B_e\leq 1-o(1)
	\end{equation}
	\dwnote{what $o(1)$ term here? what normalization} for any vertex $v$. If $\sum_{e\ni v}updated(B_e)$ satisfies  \eqref{frac-deg-exp-bound} w.h.p, then we are done. \dwnote{clean up garbage writing} We must therefore also argue some form of concentration. \dwnote{filler text}	
	\begin{align*}
	\sum_{e\ni v} UB_e & = \sum_{e\ni v} (B_e/\Pr[U_e])\cdot U_e \\
	& = \sum_{e\ni v} (B_e/\Pr[U_e])\cdot (1-\sum_{c\in S} \mathds{1}[e\in M_c])
	\end{align*}
	For any fixed color $c$ and vertex $v$, we denote the (negative) additive contribution of coloring edges of  $v$ by $c$ by
	\begin{equation}
	A_{c,v}=\sum_{e\ni v} (B_e/\Pr[U_e])\cdot \mathds{1}[e\in M_c].
	\end{equation}
	 We will show concentration of these $A_{c,v}$'s. As $\sum_{e\ni v} UB_e$ is equal to a fixed constant $\sum_{e\ni v} B_e/\Pr[U_e]$ minus the sum of these $A_{c,v}$'s, this will imply concentration of $\sum_{e\ni v} UB_e$.
	
	Now: for any $c,v$ and filtration $\mathcal{R}$\dwnote{restate} based on other $A_{c',v'}$ values for $c'>c$ in the \metaphase and $v'\in V$, we have 
	\begin{equation}\label{Acv-bound}
		\E[A_{c,v} \mid \mathcal{R}] \geq \left(\sum_{e\ni v} (B_e/\Pr[U_e]) \cdot f_{e,c} \cdot (1-o(1))\right) - O(c^{2/3-0.9}).
	\end{equation}
	\textbf{SUMMING OVER $c^{2/3}$ colors $\rightarrow$ additive error of $c^{2/3} c^{2/3-0.9}$.... TOO BIG. Reason we changed phases length to $d^{0.4}$.}
	
	\dwnote{todo: think... :-/ }
	The variables we use to lower bound $A_{c,v}$, denoted by $\widehat{A_{c,v}}$, essentially consist of the same distribution after removing some $O(c^{2/3})$ most-significant contributing edges $e$ to $A_{c,v}$...
	Similar to proof of \cref{color-concentration}, only also taking into account that $\Pr[e\in M_c] \geq f_{e,c}\cdot (1-o(1))$ if $e$ is not colored before $c$ \textbf{and $\sum_e B_e$ LARGE!!!}\dwnote{crux of argument}... 
	Since $B_e = f_{e,c'} \leq O(1/c') = O(1/c^{0.9})$ and (reason why $1/Pr[U_e]$ not too large...), we find that potentially coloring an edge $e$ before trying to round 
	color $c$ can decrease $A_{c,v}=\sum_{e\ni v} (B_e/\Pr[U_e])\cdot \mathds{1}[e\in M_c]$ by $B_e/Pr[U_e]\leq O(1/c')$. The overall contributions of these $O(c^{2/3})$ subtractions to $A_{c,v}$ are therefore at most $O(c^{2/3} /c') \leq O(c^{2/3 - 0.9})$.
	
	We now use Bernstein's inequality to argue concentration. The independent variables $\widehat{A_{c,v}}$ correspond to picking some value $B_e/\Pr[U_e]$ with probability $\Pr[e\in M_c]$. The variables $W_e = (B_e/\Pr[U_e])\cdot \mathds{1}[e\in M_c]$ are easily shown to be negatively correlated (as only one edge $e\ni v$ can be picked). Therefore, we have that the variance of this $\widehat{A_{c,v}}$ is at most the sum of variances of the independent weighted Bernoulli variables, $W_e$. Therefore, since $B_e/\Pr[U_e] = O(1/c^{0.9})$, this implies that $\VAR(W_e) \leq O(1/c^{1.8})$. As $v$ has at most $\Delta=O(c^{1.1})$\dwnote{assumption}, this implies a 
	\begin{equation}
	\VAR(\widehat{A_{c,v}}) \leq \VAR(\sum_e W_e) \leq  O(1/c^{0.7}).
	\end{equation}
	In addition, we have that $\widehat{A_{c,v}}\leq 1/c' = O(1/c^{0.9})$ always. Now, appealing to Bernstein's inequality, we find that w.h.p., $\widehat{A_{c,v}} \geq \E[\widehat{A_{c,v}}] - .$\dwnote{use Bernstein, below}	
	
	Note: plugging in $A_{c,v}$ bounds into $UB_e$, summing  over all $O(c^{2/3})$ colors, get additive error of $O(c^{4/3-0.9})$. \textbf{TODO: replace all $2/3$ with, say $0.4$.}
	
	\subsection{Still missing:}
	\begin{enumerate}
		\item \st{if sum $B_e$ is large, we're good} \dwnote{Looks like we don't need this}
		\item Bernstein on ``independent'' $A_{c,v}$'s gives concentration (generalization of 3.3 to non-binary $Y_i$). Note: Variance and realized values is SMALL for independent $A_{c,v}$.
		\item argue that $1-\Pr[U_e]$ is roughly $\sum_c f_{e,c}(1-o(1))$. \textbf{THEREFORE, $\sum_c \E[A_{c,v}]$ is essentially $\sum_{e} (B_e/\Pr[U_e])\cdot (1-\Pr[U_e])$, and we are done.}\dwnote{	
			Note that $\Pr[U_e] = 1-\sum_{c\in S} \Pr[e\in M_c] \leq 1-\sum_{c\in S} f_{e,c}$, since our \roundM algorithm loses just a little, and same for not updating...}
		\item choose numbers so that additive error is at most 1/number of \metaphase{}s (otherwise, additive error throughout is not $o(1)$).
	\end{enumerate}
\end{proof}	

\begin{lem} %[Bernstein's Inequality for NUOD Bernoulli variables]
	\label{lem:bernstein}
	Let $X_1,X_2,\dots,X_n$ be independent random variables with $\E[X_i] = 0$ for all $i$ and $X_i\leq M$ always, and let $X=\sum_i X_i$. Then,
	$$\Pr[X > \E[X] + a] \leq \exp\left(\frac{-a^2}{2(Var(X) + aM/3) }\right).$$
\end{lem}



\textbf{If $\sum_{e\ni v} \sum_{c\in \metaphase} f_{e,c}$ is small -- no worries. Must have many \metaphase{}s where it is large if you have high degree. (If don't have high degree, don't care.)}



\begin{lem}\label{update-concentrated}
	$\sum_e UB_e\geq \sum_e B_e - o(1)$ w.h.p. \dwnote{careful: don't accumulate! Pick $o(1)$ carefully}
\end{lem}
\begin{proof}
	Upper bound from above. 
	Other direction: similar argument, noting that our \roundM guarantees $\Pr[e\in M_c]\leq f_{e,c}$.
\end{proof}	

By \Cref{frac-deg-concentration} our \roundM algorithm always outputs 
Combining \cref{color-concentration}, \Cref{frac-deg-concentration} and the \Cref{update-concentrated} we find that we color all but a $o(1)\cdot \sum_{e,c} f_{e,c}$ fraction of $v$'s edges w.h.p, and so \Cref{line:greedy} only incurs an extra $o(\Delta)$ colors w.h.p., implying our main result.

\begin{thm}
	Let $f$ be a $c$-competitive fractional edge coloring with \textbf{PROPERTIES}.... Then, there exists a \roundEC which outputs a $c(1+o(1))$-competitive edge coloring w.h.p.
\end{thm}


\subsection{Use of Meta-Phases}



... This will allow us to argue that the effect of edges being colored by some color $c$ during the meta-phase should not affect the probability of matching an edge for subsequent colors in the meta-phase by too much.
For this, we need to argue first that the updated values are not too large. While this is not true for all fractional edge colorings, we will modify our fractional edge colorings slightly in order to guarantee this is the case.
Specifically, for any edge $e$, let $c(e)$ be the lowest color such that $\sum_{c=1}^{c(e)} f_{e,c} \geq \frac{1}{\Delta_e^{1/5}}$, where $\Delta_e$ is the maximum degree upon arrival of edge $e$. 


\begin{obs}\label{cap-P} 
	Replacing all $f_{e,c}$ by zero for all $c\leq c(e)$ only decreases $\sum_{c} f_{e,c} = 1$ by a $1-o(1)$ multiplicative term.\dwnote{pick correctly to make next corollary work...}
\end{obs}

We will work with these modified values, possibly causing us to leave some $o(1)$ fraction of the edges of $v$ unmatched by the end of the algorithm in expectation...

\begin{cor}\label{cap-updated}
	For a fractional solution satisfying $f_{e,c}\leq 1/\Delta_e (\leq 1/c)$ for all $(e,c)$, we have that if we modify each edge as in \Cref{cap-P}, then $\textrm{\emph{updated}}(f_{e,c}) \leq \frac{1}{\sqrt{c}}$.\dwnote{have to be at most roughly $1/c$...}
\end{cor}
\begin{proof}
	Let $f_{e,c}$ be the values assigned to the edges after this modification. Then, we find that
	\begin{align*}
	\textrm{updated}(f_{e,c}) & \leq  f_{e,c}/(1-P_{e,c+1}) \\
		& \leq f_{e,c}/(1-\sum_{c'> c} f_{e,c}) \\
		& \leq f_{e,c} / (\frac{1}{\Delta_e^{1/5}}) \\
		& \leq \frac{1}{\Delta_e^{4/5}} \\
		& \leq \frac{1}{c^{4/5}},
	\end{align*}
	where the second to last inequality follows from the hypothesis, whereby $f_{e,c}\leq \frac{1}{\Delta_e} \leq \frac{1}{c}$.\dwnote{Bound $\Pr[U_e]$....}
\end{proof}

Now, consider some vertex $v$. By the above, we find that during a meta-phase of length $c^{2/3}$, starting with color $c\geq XXXX$,
the set of edges of $v$ colored during the meta-phase contribute at most $c^{2/3}\cdot 1/c^{4/5} = 1/c^{2/15}$ to any $F_{c'} \triangleq \sum_{e} \textrm{\emph{updated}}(f_{e,c'})$ for all colors $c'$ in the meta-phase.
Let 
$F \triangleq \sum_{c'\in \textrm{meta-phase}} F_{c'}$ be the overall updated values of edges of $e$ and colors for this meta-phase. If $F\leq c^{1/2} = c^{2/3}/c^{1/6}$, we don't mind not receiving anything during this phase (such phases will invariably account for at most a $1/c^{1/6}$ fraction of the overall....\dwnote{overall what?} If however this value is at least $c^{1/2}$, we find that the change to $F$ by assuming 


\subsection{To Show:}
\begin{enumerate}
\item Above argument proves that we can lower bound the probability of matching in a particular phase (where the updated values are high) by some $(1-o(1))$ times their value and show that this ALWAYS lower bounds the probability of matching an edge of $v$ for a given color. Coupling then implies the number of colored edges is at least its expectation times $(1-o(1))$ minus some $o(c^{2/3})$ term w.h.p.
\item $\sum_{e,c\in meta-phase} \textrm{\emph{updated}}(f_{e,c})$ is sharply concentrated around its mean.
\item Putting both together yields good bounds.
\end{enumerate}

%\begin{obs}
%	If $f_{e,c}\leq 1/c$ for all $c$, and $c_{\max} \leq C\cdot \Delta$ for some constant $C\geq 1$, then the probability of $e$ being colored by color $c$ or greater is at most $P_{e,c}\leq H_{\Delta} - H_{c} \leq \ln(\Delta/c)$.
%\end{obs}
%
%
%\dwnote{NOTE: we rely on $f_{e,c}\leq 1/c$ for all edge-color pair $(e,c)$}

Let $v$ be some high degree vertex.
We now argue that conditioned on a particular set of edges of $v$ being uncolored at the beginning of a super-phase, each of the edges 


This is not quite so simple, as clearly the 
For this to work we need to also argue that only updating the values $f^{(c)}$



Now, obtaining $\widehat{P}_{e,c}$ as above


\begin{thm}\label{rounding-result}
	Let $\{f_{e,c} \mid e\in E,\, c\in \mathbb{N}\}$ be a fractional edge coloring revealed online such that for each edge-color pair $(e,c)$ we have $f_{e,c}\leq \frac{1}{c}$. Modifying $\vec{f}$ as in \Cref{cap-P} guarantees that by \Cref{line:greedy} all but $o(\Delta)$ edges of each vertex are colored, w.h.p.
\end{thm}

Finally, having described our approach for rounding online edge coloring (i.e., presenting an \roundEC) and analyzed it, we are finally ready to prove our main results for randomized online edge coloring. Both theorems are a direct corollary of \Cref{rounding-result}, as the optimal online fractional solutions for known $\Delta$ (assign $1/\Delta$ to each edge) and the coloring given by \Cref{alg:cap_water_filling} both assign small values to all edge-color pairs (the latter algorithm assigns values of at most $1/\log^{\logbound} n$). As such, our \roundEC rounds these fractional solutions online with a multiplicative loss of at most XXXXXXX=o(1), which implies our following results.

\begin{thm}
	For online edge coloring bipartite graphs, there exist $(1+o(1))$-competitive randomized algorithms if $\Delta=\Omega(\log^{\logbound} n)$ is known.
\end{thm}
\begin{thm}
	For online edge coloring bipartite graphs, there exist $\left(\frac{e}{e-1}+o(1)\right)$-competitive randomized algorithms if $\Delta=\Omega(\log^{\logbound} n)$ is unknown.
\end{thm}
